A blockchain-based e-goverment service for Quantity Surveyors

In Spain, quantity surveyors are entitled to carry out official cadastral surveys, attestations, and certificate issuing according to a well-defined professional code. Official Associations of Quantity Surveyors and Technical Architects (COAAT) are responsible for endorsing the documentation related to actions performed on buildings. An e-platform that enables immutability, traceability, and a unique property record among all the Spanish COAATs, with an affordable cost, is essential to streamline the involved processes. The blockchain technology and smart contracts have recently emerged as promising solutions for e-government services due to the inherent features provided by the technology. In this paper, we identify the design goals and propose a blockchain-based e-government system for the electronic management of the documentation generated, submitted, and validated by the Spanish COAATs, namely, the COAATChain. The proposal has been deployed and evaluated on the Binance testnet blockchain, in order to assess its affordability.

==> OLDintro.tex <==

%\label{sec:introduction}


\mbc{explicar Problem relevance G2, Research contributions G4 ---> research questions; G6: design as a search process---> la tecnología blockchain es la adecuada para cubrir requistos no funcionales del sistema ---> CAMBIAR EL DISCURSO --> PARTIR DE EXPLICAR EL PROBLEMA Y ENLAZAR CON LA TECNOLOGÍA QUE DA LAS CLAVES PARA SOLUCIONARLO???}

\cce{Reordenar para dejar aquí solo problem statement G2 (primeros párrafos), el context (1 párrafo de seccion system requirements para contar a running case) and objective/contribution G4}

\cce{añadir luego una especie de related work  bajo el nombre: blockchain-based e-goverment services con los párrafos de previous research}

\chapterinitial{All over the world,} governments and government agencies are now implementing projects and initiatives for digital transformation and to provide effective digital services or e-government~\cite{ebsi}. 
In general, e-government services improve citizen experience and save costs. 
Users expect a high-availability and fault-tolerance from the e-government service which increase its satisfaction. Nowadays, emerging technologies and innovative practices help governments to meet these requirements.
In particular, blockchain-based smart contracts are one of the most up-and-coming solutions with significant features for e-government services~\cite{HEWA2021}.


Blockchain technology is based on anonymous peer-to-peer transactions, without any centralized control~\cite{nakamoto2008bitcoin}. Smart contracts are digital programs whose codes are stored on the blockchain. These programs are immutable, self-verifying and self-executing digital contracts~\cite{ferdous2020blockchain}. 
Hence, smart contracts driven by blockchain guarantee that transaction processes are time-efficient,  cost-effective 
and secure compared to conventional contracts
without requiring the intervention of third-party intermediaries~\cite{ali2019survey}.



\cce{los párrafo que vienen a continuacion Identify previous research on the topic..a otro lado??..}

Smart contracts are applicable in different application domains (i.e. financial applications, e-government, currency management, banking industry, insurance,  auditing procedures or healthcare domain).
Most of the proposed blockchain solutions are at an early stage, as only a small set of them have progressed to the system evaluation phase or even to the prototype deployment phase~\cite{Lykidis2021}.

Within the e-government domain, we find blockchain-based solutions for electronic voting system which ensure authentication, anonymity, accuracy, and verifiability~\cite{garg2019comparitive}, or distributed ledger based approaches to automate the intellectual property licensing payments~\cite{Tietze2020}. 
We also find modeling for the semi-automated translation of human-readable contract representations into computational equivalents that enable the encoding of laws~\cite{frantz2016institutions}.
In~\cite{chiang2018exploring}, the authors present ChainGov as a collaborative blockchain and smart contract integrated platform to build the trust between  immigrants, governments, and other institutions informing about the flow of money as well as real time visibility of all transactions. 
Also, blockchain has been proposed as the core to support global vaccination strategies for COVID19, harnessing its decentralization and global unique identification~\cite{Costa2022}.
Moreover, the European Commision is building its own blockchain infrastructure, the European Blockchain Services Infrastructure (EBSI), \emph{``to leverage blockchain to create cross-border services for public administrations, businesses, citizens and their ecosystems to verify information and make services trustworthy''}~\cite{ebsi}. EBSI focuses on providing verifiable credential services, and traceability of documents, among others. There are several ongoing pilot projects to demonstrate its usefulness and increase awareness and adoption of the technology.

\cce{Identify objetive (OB) and research questions (RQ): 
¿ se puede usar una DApp para mejorar la gestion realizada por COAAT?
RQ: supone fijarse en una serie puntos o propositions (What particular (causal) relationships are to be investigated? )---> entiendo que son los puntos enumerados en nuestros requerimientos: decentralized, immutable, property, trace, cost
}

\deli{[¿En este párrafo proponer el artefacto que queremos realizar? Que básicamente es lo que hemos comenzado a decir.]}\hl{This paper develops an e-government system for the electronic management and distribution of the documentation generated, submitted and validated by an official association of quantity surveyors. To the authors' best knowledge, no previous work has been done in this e-government service. Note that the Spanish Official Association of Quantity Surveyors and Technical Architects (COAAT, by its Spanish acronym) is in charge of endorsing the documentation of the projects, referring to new building works, refurbishments or energy efficiency in order to grant them an additional validity for their subsequent presentation to public bodies, administrations, city councils or community boards. Surveyors carry a lot of responsibility according to a well-defined professional code. For example, they carry out official cadastral surveys and may perform attestations and issue certificates. Some types of projects, such as building demolitions, require mandatory approval by a COAAT.}

\subsection{System Requirements \mbc{--> Problem description? Current-state analysis??}}

\mbc{[ G1 (design as an artifact) ---> definir requisitos que se tendrán en cuenta al diseñar el artefacto]}

\deli{[Yo aquí veo que dandole una pequeña vuelta se puede describir la relevancia de la solución G2 y el diseño de la evaluación G3?}

\deli{En el párrafo siguiente (resaltado en azul), que ya se hace, se describiría el estado actual del sistema y sus problemas, más formalmente.]}
\sethlcolor{cyan}
\hl{For many years it was compulsory to present all the physical documentation in person at the offices of the professional associations, leave it for a few days for review and validation is appropriate, 
then collect the approved documentation and finally present it to the corresponding public administration. It should be noted that each professional association represents a demarcation, which coincides with the provincial administrative division. There may be several professional associations in a country.

In recent times, both professional associations and public administrations have made technological efforts to digitise this process. For example, the digital certificate system is now supported, which saves time and travel.
However, there are still some important challenges and requirements for improvement, such as, for example: }

\begin{itemize}
\item \hl{Decentralized and fault-tolerant system: Use a distributed architecture to get a high availability even when some nodes fail.}
\item \hl{Immutability: Prevent manipulation of property records by a central authority or a third party.}
\item \hl{Common and unique property record: Avoid double property records and share information among different official associations.}
\item \hl{Record traceability, timestamp and provenance: Keep track of property records.}
\item \hl{Cost reduction: By automatizing and streamlining the access, processing and validation of property records.}
\end{itemize}


In this paper, we develop a decentralized application and designed an e-government system for the Spanish Official Association of Quantity Surveyors and Technical Architects.  
Note that the files and documents submitted to the platform will be reviewed by a COAAT,
which is the competent authority in charge of granting the approval.  
In case of irregularities, such as the existence of technical errors or the duplicity of a dossier, validation will be denied. Then, the corrected documents may be resubmitted. 
All verified documents will be assigned a SVC (Secure Verification Code) that will be used for subsequent verification by other involved agents. 

\deli{[Aquí describimos los beneficio, la relevancia, de nuestra solución]}
\definecolor{lightred}{rgb}{1,0.95,0.95}
\sethlcolor{pink}
\hl{Incorporating blockchain technology in this platform guarantees the immutability, verification and traceability of the documents by third parties, such as public administrations, courts, notaries, construction promoters or individuals themselves. Moreover, this technology ensures a decentralized fault-tolerant architecture without single points of failure.}
%, and also providing immutability. 
\hl{So, this e-government proposal, besides saving on paper, cuts management costs, streamlines processes, and provides accurate and reliable information on properties. In summary, the contributions of the paper are as follows.}

\deli{[No tanto especificar las contribuciones, sino la lista de soluciones que proponemos a los problemas que antes hemos detallado en el párrafo en azul]}

    \textbf{-}  \hl{Design of an electronic protocol for the governance of the tasks performed by the Official Association of Quantity Surveyors and Technical Architects. Specifically, to generate, verify and consult the documentation generated by them, guaranteeing its immutability and traceability.}
    
    \textbf{-} \hl{Implementation of the proposed electronic governance protocol, called COAATChain, on a blockchain-based platform,  incorporating distributed storage capacity. Additionally, a simple DApp has been implemented for testing purposes.}

\deli{[Esto me lo llevaría a la sección de evaluación]} \sethlcolor{lime}\hl{The approach has been deployed and evaluated on the Binance testnet blockchain. As a result of harnessing the blockchain technology, immutability and traceability have been achieved and also a significant reduction in management time at a reduced economic cost.}

The rest of the paper is organized as follows. First, we introduce COAATChain as a distributed blockchain-based platform for e-government support of the COAATs, and also describe the operation model of the proposed protocol. Then, a cost analysis of the approach is discussed. And finally, conclusions and future work are presented.





==> intro.tex <==
%progem statement G2
\chapterinitial{All over the world,} governments and government agencies are now implementing projects and initiatives for digital transformation and to provide effective digital services or e-government~\cite{ebsi, estonia}. 
In general, e-government services improve citizen experience and save costs. 
Users expect high-availability and fault-tolerance from the e-government service which increase their satisfaction. 
Nowadays, emerging technologies and innovative practices help governments to meet these requirements.
In particular, blockchain-based smart contracts are one of the most up-and-coming solutions with significant features for e-government services~\cite{HEWA2021}.

%centro tema
In this paper, we will focus on the Spanish Official Association of Quantity Surveyors and Technical Architects (COAAT, by its Spanish acronym) which is in charge of endorsing the documentation of the projects, referring to new building works, refurbishments or energy efficiency in order to grant them an additional validity for their subsequent presentation to public bodies, administrations, city councils or community boards. Surveyors carry a lot of responsibility according to a well-defined professional code. For example, they carry out official cadastral surveys and may perform attestations and issue certificates. Some types of projects, such as building demolitions, require mandatory approval by a COAAT.

%This paper develops an e-government system for the electronic management and distribution of the documentation generated, submitted and validated by an official association of quantity surveyors. 
%To the authors' best knowledge, no previous work has been done in this e-government service. 
%Note that 
%estado actual; relevancia de la situación
% G1 requisitos

%Estado actual % AS IS analysis
For many years it was compulsory to present all the physical documentation in person at the offices of the professional associations, leave it for a few days for review and validation if appropriate, then collect the approved documentation and finally present it to the corresponding public administration. It should be noted that each professional association represents a demarcation, which coincides with the provincial administrative division. There are several professional associations within a country.
In recent times, both professional associations and public administrations have made technological efforts to digitise this process. For example, the digital certificate system is now supported, which saves time and travel.
However, there are still some important challenges and requirements for improvement. 

A digital service for the Spanish COAAT should tackle the following outstanding features:
%goals: 
%first level goals (FLGs):
%problema a resolver
%develop a decentralized application and design an e-government system for the Spanish Official Association of Quantity Surveyors and Technical Architects that addresses the points mentioned above by using the blockchain technology.  

\begin{itemize}
%\item Decentralized and fault-tolerant system: Use a distributed architecture to get a high availability even when some nodes fail.
\item Immutability: Prevent manipulation of property records by a central authority or a third party.
\item Common and unique property record: Avoid double property records and share information among different official associations.
\item Record traceability, timestamp and provenance: Keep track of property records.
\item Affordability: Automate and streamline the access, processing and validation of property records at reduced cost.
%\item Cost reduction: By automatizing and streamlining the access, processing and validation of property records.
\item Resiliency: Provide a system setup with high availability and fault-tolerance.
%eso gracias a esto : ) Use a distributed and decentralized architecture to get a high available and fault-tolerant system.
\end{itemize}

%------------------
%\cce{reescribir estos párrafos}

%\cce{Research question ????}

%And, as a solution of the paper are as follows.
%Each of the goals mentioned above are related with a researh questions.  

%solucion???
Having into account the current-state analysis, our main objective is to design a decentralized e-government system for the Spanish COAAT that fulfils the key features mentioned above.
In a nutshell, our proposal uses the following solutions:

\begin{itemize}
    \item The design of an electronic governance system, called COAATChain, based on role definitions. % and smart contracts.
    \item The implementation of the system with smart contracts.
 
 \end{itemize}
%\cce{SOLUCION..usar BC}

A methodology similar to the T-DM methodology proposed in~\cite{udokwu2021} has been followed to derive the system implementation from the system value proposition. As a result, the COAATChain system has been designed, deployed and tested on a blockchain-based platform to meet the initial requirements.

%------------------
The rest of the paper is organized as follows. First, we present the related work. We then introduce COAATChain stakeholders and its first level goals (FLGs), and also describe the most important implementation details. Then, a design evaluation of the approach is discussed. And finally, conclusions and future work are presented.
 

\section{Related work}

%Smart contracts are digital programs whose codes are stored on the blockchain. These programs are immutable, self-verifying and self-executing digital contracts~\cite{ferdous2020blockchain}.

Smart contracts are digital programs whose code is stored on the blockchain~\cite{ferdous2020blockchain}. These programs are applicable in different application domains (i.e. financial applications, e-government, %currency management, banking industry, 
insurance, auditing %procedures 
or healthcare). % domain).
%Most of the proposed blockchain solutions are at an early stage, as only a small set of them have progressed to the system evaluation phase or even to the prototype deployment phase~\cite{Lykidis2021}.

Within the e-government domain, we find blockchain-based solutions for electronic voting which ensure authentication, anonymity, accuracy, and verifiability~\cite{garg2019comparitive}, or distributed ledger based approaches to automate the intellectual property licensing payments~\cite{Tietze2020}. 
We also find modeling for the semi-automated translation of human-readable contract representations into computational equivalents that enable the encoding of laws~\cite{frantz2016institutions}.
In~\cite{chiang2018exploring}, the authors present ChainGov as a collaborative blockchain and smart contract integrated platform to build the trust between immigrants, governments, and other institutions informing about the flow of money as well as real time visibility of all transactions. 
Also, blockchain has been proposed as the core to support global vaccination strategies for COVID19, harnessing its decentralization and global unique identification~\cite{Costa2022}.
\hl{One of the countries that have advanced most in terms of e-government is Estonia~}\cite{estonia}. \hl{They have created the concept of digital country, where many procedures can be carried out by electronic means. In particular, an ad-hoc scalable blockchain was developed to ensure integrity of data stored in government repositories and to protect its data against insider threats.} %But no information regarding the specific use case we address has been found. 
%\cce{falta referencia del primer reviso!!!!}

Moreover, the European Commision is building its own blockchain infrastructure, the European Blockchain Services Infrastructure (EBSI), \emph{``to leverage blockchain to create cross-border services for public administrations, businesses, citizens and their ecosystems to verify information and make services trustworthy''}~\cite{ebsi}. EBSI focuses on providing verifiable credential services, and traceability of documents, among others. There are several ongoing pilot projects to demonstrate its usefulness and increase awareness and adoption of the technology~\cite{Lykidis2021}.
%Most of the proposed blockchain solutions are at an early stage, as only a small set of them have progressed to the system evaluation phase or even to the prototype deployment phase~\cite{Lykidis2021}.


==> life-cycle.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.7\textwidth]{./figs/esquema-general-sistema.jpeg}
    \caption{High-level design of smart contract in COAATChain.}
    \label{fig:structureCOAAT}
\end{figure*}

The usual life cycle of the system could be as follows (see Figure~\ref{fig:structureCOAAT}). The system administrator (\textit{Role~0} stakeholder) deploys the main smart contract (\textit{Set up system}, \textit{Step $1$}), and registers each of the \textit{Role~1} stakeholders (\textit{Add COAAT, step $2$}). These steps are carried out using the \textit{Role~0} stakeholder wallet address of the blockchain network on which the system is deployed. Then, the COAATs will be able to register their corresponding \textit{Role~2} and \textit{Role 3} (\textit{Add users, step $3$}).

At this point, a \textit{Role~2} stakeholder registered in the system will be able to deploy a new smart contract associated with a property (\textit{Add new property, step $4$}), including all its necessary information (i.e. cadastral reference, surface area, address, etc.).  Then, the \textit{Role~2} stakeholder will be able to add a new dossier on a property (\textit{Add new dossier, step $5$}), which may include one or several files (\textit{Add file to dossier, step $6$}, further details on this are given later). Note that to include a new dossier it is mandatory that the property to which it belongs is already registered. Therefore, if the system detects that the associated property does not exist, the \textit{Role~2} stakeholder will be required to register the property beforehand.

It must also be taken into account that it is not possible to have more than one open dossier per property. Consequently, before registering a new dossier, the smart contract checks that there is none open. Once a property has been registered in the system and all of its associated files have been closed, the \textit{Role~2} stakeholder will be able to view the registered files and also register new ones. 

A dossier incorporates basic data such as dossier type or budget, and will sometimes require the inclusion of additional documentation with a higher storage cost (e.g. digitally signed files in PDF format). These files are the ones that will be validated or rejected by the COAAT technicians (\textit{Role~1} stakeholder), and therefore it is necessary to store them in the system. As pointed out above, IPFS is harnessed for the distributed storage of these files. So, the blockchain will store only the CID (Content IDentifier) and SVC (Secure Verification Code) to unambiguously identify the files associated with a dossier. While the CID is generated by the IPFS to access the file stored in it, the SVC is generated by COAATChain for each of the files attached to the dossier. Thus, each pair (CID, SVC) is unique for each file, and is used to search and locate the concerned file.

In this way, to add a file to a dossier (\textit{Add file to dossier, step $6$}), \textit{Role~2} stakeholder accesses the dossier using the cadastral reference associated to the property and calls the ``Add File to Dossier'' function. This function will open a form with a newly generated SVC, which is included in the PDF file. Then, the file will be digitally signed and uploaded to the IPFS system, which will return its CID code. Finally, the resulting CID code is automatically added into the form opened by the smart contract function. Note that the use of CIDs by the system is fully transparent to users, with the system internally managing both their inclusion and their reading from the blockchain. 
Once all the documentation has been added to a dossier, a \textit{Role~2} stakeholder may request its validation from the COAAT (\textit{Role 1} stakeholder). This will cause the smart contract to generate an asynchronous event that will alert the COAAT to proceed to validate the concerned file(s). 

In the (\textit{Validate dossier, step $7$}), the \textit{Role~1} stakeholder will be able to access all the documentation of the dossier associated with the event received from a Quantity Surveyor. Obviously not directly, but using internally the CIDs stored in the dossier, it is possible to access the IPFS and obtain the documentation. As already mentioned, this read access and the use of the CIDs is completely transparent to the user. If the documents are correct, the \textit{Role 1} stakeholder will validate them by executing the ``Validation'' function of the smart contract associated to the property. This function will generate a new SVC that will have to be added to the document as a verification proof. Once digitally signed, the verified document will be automatically uploaded to the IPFS, storing its CID in the blockchain thanks to the ``Validation'' function. This function will also generate an event to inform the Quantity Surveyor responsible for the dossier about its new status.

Once a dossier has been validated, external agents (\textit{Role~3} stakeholders) can access any documentation associated with the dossier by simply using the validation SVC (\textit{See dossier, step $8$}), which must be provided to them (i.e. by e-mail or letter). They will use the SVC in the platform to locate the document, which could be download in order to check it out.


==> xxxxxCOOATChain-system.tex <==
%\section{Stakeholders and system value proposition}

Different stakeholders (i.e., user roles) have been identified for the proposed COAATChain system, based on expert knowledge. These are the following:

\begin{itemize}
    \item \textbf{Role~0 (System Administrator)}: Responsible of the initial deployment of the system and the registration of the COAATs.
    
    \item \textbf{Role~1 (COAATs)}: They can access, validate or reject dossiers. They can also register new properties by deploying their associated smart contracts. Additionally, COAATs are in charge of registering quantity surveyors (Role~2), and other agents (Role~3). 
    
    \item \textbf{Role~2 (Quantity Surveyors and Technical Architects)}: They can register a new property, create a new construction dossier associated to an existing property, and include documentation to the dossiers previously created by them. A quantity surveyor cannot access the dossiers created by other surveyors, even though he/she can see that they exist.
    
    \item \textbf{Role~3 (Read-only users)}: %mbch: SIMPLIFICO These users will only be able to view the documentation %through the use of the SVC associated to the document they wish to view. They will be
    Notaries, courts, public administrations, and any legal entity that by law has the right to access the information in the construction dossiers stored in the system. 
\end{itemize}


%cce cuidado con el ingles...dos also seguidos y el pare´ntesis que dice que se verá mas en la seccion,eh?. 
As outlined in previous sections, the main value proposition of COAATChain (see Figure~\ref{fig:COAAT-svp-flg}) is \textbf{to provide a distributed e-government architecture for Spanish COAATs}. As the platform harnesses the blockchain technology, it inherits its main features, namely, \emph{immutability}, \emph{traceability} and \emph{resiliency}. Also, \emph{affordability} will be ensured due to the relatively low fees introduced by the use of blockchain platforms (more on this in Section ``Design evaluation'')%mbch no sé porqué no se coge el número de sección al compilar... quizás al estar en otro fichero?
, but also because the proposed solution is engineered to keep the amount of information stored in the blockchain to the minimum, while also guaranteeing the immutability, traceability and accessibility of the documentation.

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=1.0\textwidth]{./figs/SVP-and-FLG-model.jpg}
    \caption{COAATChain system value proposition and its FLG model.}
    \label{fig:COAAT-svp-flg}
\end{figure*}

%cce ...ingles??  assigned task to each stakeholder %mbch no es que se asignen, es lo que cada usuario debe poder hacer una vez esté hecho el sistema
From the main value proposition and the tasks every stakeholder must be able to accomplish, the first level goals (FLGs) of the COAATChain platform have been derived in Figure~\ref{fig:COAAT-svp-flg}. 
The \emph{System kick-off} goal deploys the system on the selected blockchain platform. 
The \emph{Add new COAAT} goal enables the addition of new COAATs into the system (recall that there is usually a COAAT per province in Spain, and there are also Regional COAATs). 
The \emph{Add new user} goal provides the capability of creating the remaining user roles in the system (on one hand, quality surveyors and technical architects, and on the other hand, read-only users). % MBCH--> se dice después...These latter two goals might involve the execution of Know Your Client (KYC) strategies to verify the identities of the new users. 
The \emph{Register new property} goal inserts the details of a property into the system. Properties can be associated to one or more dossiers, while only one of them might be open at a certain moment. 
The \emph{Manage dossier} goal enables the inclusion of a new dossier into the system, as well as the addition of properties and documentation associated to it. 
The \emph{Validate dossier} goal is one of the critical goals of the system, because only the COAAT stakeholder can validate (or not) the dossier, after examining its associated documentation. 
Lastly, the \emph{View document} goal enables the visualization of the documentation held by any COAAT by generic, authorized read-only stakeholders.

Most relevant quality goals have also been identified per every FLG in Figure~\ref{fig:COAAT-svp-flg}. These represent the non-functional system properties associated to each of them. The quality goal \emph{affordable} refers to the feasibility that deployment costs can be assumed by the COAATs. \emph{Secure} means that there will be controls to prevent unauthorized manipulation of certain assets. Finally, the main aim of the system is to enable \emph{transparent} access to documentation for authorized stakeholders.
Moreover, the quality goals associated to the main value proposition (namely, \emph{immutable}, \emph{traceable}, \emph{resilient}, \emph{affordable}, discussed above) are inherited by all the FLGs derived from it. 

Finally, the different FLGs have been assigned to their corresponding stakeholder, following the detected actions that each of them is required to perform. For example, Role 3 stakeholders (RO Users) are only associated to the goal \emph{View document} while  Role 1 stakeholders (COAATs) are associated to three goals: \emph{Add new user (Role 2, 3)}, \emph{Validate dossier} and \emph{Register new property}.

\subsection{FLG implementation details}
%mbc quito colorines para ir limpiando el documento, cuando revisemos el texto casi definitivo los volvemos a usar
\hl{Stakeholders are uniquely identified in the blockchain network thanks to their wallet address. A Know Your Client (KYC) agent, in order to assess the identity of the stakeholder responsible for the wallet, should be deployed. Each wallet address is associated with the corresponding role according to the type of stakeholder. In addition, access to FLGs is pre-validated by implementing ``modifiers'' that check the role of the user trying to execute that function.}

The \emph{System Kick-off} goal consists of the deployment on the blockchain platform of the \textbf{contract factory} that will implement the FLGs \emph{Add new COAAT}, \emph{Add new user} and \emph{Register new property}.

%\cce{relacionar esto con el diagram de secuencia ??}
%\cce{quizá se puedan entre mezclar las frases marcadas en rojo con lo que hay detrás sobre el contract factory y así para el property contract}
%\cce{ si, creo que se repite, unimos partes: este párrafo que viene es parecido a "Then, the following FLGs are implemented by
%means of the contract factor"...juntamos ponemos estos detalles de implementacion de una}

The \emph{Add new COAAT} and \emph{Add new users} goals consist of the identification through a reliable and secure KYC strategy of the new user to be included in the system. Their wallet address as well as identifying data will be included in the blockchain along with the assigned role.

The \emph{Register new property} goal is implemented as a method on the contract factory that should be executed by a Role 1 or Role 2 stakeholder. A transaction deploying a new smart contract for that property, i.e., the \textbf{property contract}, is issued. The cadastral data of the new property must be provided at contract deployment for identification purposes. This smart contract will implement all the FLGs associated to that property, namely, \emph{Manage dossier}, \emph{Validate dossier} and \emph{View dossier}.
The \emph{Manage dossier} goal implies entering all the data related to the new dossier into the system, as well as the additional documentation required for its validation by the COAAT. This additional documentation is provided in digitally signed PDF files. To implement \emph{immutability} and \emph{security} in the handling of these files, the system generates a SVC (Secure Verification Code) for each of them. This code must be included by the user in the PDF file before signing it digitally. \hl{These files are digitally signed by a nation-wide certification entity, more precisely, certificates issued by the ``F\'abrica Nacional de Moneda y Timbre (FNMT)'' (National Mint and Stamp Office) are used}\footnote{\hl{The FNMT root certificates can be downloaded from} \url{https://www.sede.fnmt.gob.es/descargas/certificados-raiz-de-la-fnmt}}.
One of the main issues to support the design goals of COAATChain is the creation of a common database for all COAATs, to avoid duplication of documentation and unify access to system resources. This is accomplished by means of the blockchain technology. However, PDF files are not saved in the blockchain, given the high number of resources involved. Instead, they are stored off-chain in IPFS (InterPlanetary File System)~\cite{IPFS,IPFScite}. What is stored on the blockchain for each PDF is the unique CID (Content IDentifier) returned by IPFS, along with the SVC of the file. This strategy contributes to achieve the \emph{affordability} quality goal. \hl{Please note that the contents stored in IPFS (i.e., the PDF files) are public according to Spanish law.}
Figure~\ref{fig:dsecCOAAT} illustrates by means of a sequence diagram the interaction among the incumbent entities when performing the actions associated to these roles. Dotted lines represent transactions stored into the blockchain with an associated cost (fees).

%\cce{si ponemos el diagrama de secuencia, habria que ligar el texto al diagrama o al reves, no??}

The \emph{Validate dossier} goal is triggered when a Role 2 stakeholder requests a dossier validation by means of the pertinent call to the Property contract, as illustrated in Figure~\ref{fig:dsecCOAAT2}. Then, an event is sent to a Role 1 stakeholder, who will be access the dossier metadata in the blockchain, and retrieve its associated documentation from IPFS by using the appropriate CIDs. Once the documentation is processed, the dossier can be either validated or rejected, and new SVCs are included in the PDFs before signing them digitally again. The transaction on the blockchain validating or rejecting the dossier will include the CIDs returned by IPFS when the PDFs are stored in it. %\mbc{DUDA: DEBERÍA HABER UNA NUEVA INTERACCIÓN CON IPFS TRAS VALIDAR (O NO) EL DOSSIER?? }\deli{SÍ, PERO ESO IMPLÍCITAMENTE ESTÁ EN LA FRASE ANTERIOR: "The transaction on the blockchain ...." QUIZÁS SE DEBERÍA INCLUIR "} \mbc{me refiero a que faltaría una flecha en el diagrama de secuencia}\deli{SÍ FALTARÍA ESA INTERACCIÓN CON EL IPFS EN EL DIAGRAMA }
The system implements asynchronous events to alert the stakeholders with Role 1 and 2, respectively, of the inclusion of a dossier in the system and of the dossier status change.

The \emph{View document} function will allow Role 3 stakeholders to access the documentation of a validated dossier by using the SVC code associated to this document by the FLG \emph{Validate dossier}. 
The SVC code is provided to the user through any digital or traditional mechanism (i.e., e-mail or letter).


%MBC creo que esto está explicado arriba más breve In order to be able to address the affordability quality goal, some considerations must be taken regarding document storage. One of the main issues to support the design goals of COAATChain is the creation of a common database for all COAATs, to avoid duplication of documentation and unify access to system resources. This is accomplished by means of the blockchain technology. However, storing a PDF file on the blockchain generates a transaction that, on the one hand, would require a lot of mining or validation time, and on the other hand, would increase the transaction fees (gas, in the case of Ethereum). To address these constraints, the PDF files will be stored off-chain. This will also prevent the blockchain size from growing so fast. More precisely, COAATChain harnesses IPFS (InterPlanetary File System). IPFS is a distributed, peer-to-peer, content-addressable storage network~\cite{IPFS,IPFScite}. The files stored in the IPFS system are accessible through a unique CID (Content IDentifier). Hence, in our proposal, the CIDs will be incorporated into COAATChain to identify the documentation associated to each transaction. This will allow COAATs to have access to all the information generated by each of them.

%MBC está arriba Regarding stakeholders, they are uniquely identified in the blockchain network thanks to his/her wallet address. A Know Your Client agent, in order to assess the identity of the stakeholder responsible for the wallet, should be deployed. Each wallet address is associated with the corresponding role according to the type of stakeholder. In addition, access to the functions of each smart contract is pre-validated by implementing ``modifiers'' that check the role of the user trying to execute that function.

%\subsection{The life cycle of the COAATChain}

%\input{life-cycle.tex}


\begin{figure}[t]
    \centering
%    \includegraphics[width=\textwidth]{./figs/COAAtChain-diag-sec.png}
    \includegraphics[width=0.52\textwidth]{./figs/COAAtChain-diag-sec-creardossier.pdf}
    \caption{Sequence diagram - Register new property and create dossier}
    \label{fig:dsecCOAAT}
\end{figure}

\begin{figure}[t]
    \centering
%    \includegraphics[width=\textwidth]{./figs/COAAtChain-diag-sec.png}
    \includegraphics[width=0.52\textwidth]{./figs/COAAtChain-diag-sec-dossiervalidation.pdf}
    \caption{Sequence diagram - Validate dossier}
    \label{fig:dsecCOAAT2}
\end{figure}
